A Survey on Complex Tasks for Goal-Directed Interactive Agents

Goal-directed interactive agents, which autonomously complete tasks through interactions with their environment, can assist humans in various domains of their daily lives. Recent advances in large language models (LLMs) led to a surge of new, more and more challenging tasks to evaluate such agents. To properly contextualize performance across these tasks, it is imperative to understand the different challenges they pose to agents. To this end, this survey compiles relevant tasks and environments for evaluating goal-directed interactive agents, structuring them along dimensions relevant for understanding current obstacles. An up-to-date compilation of relevant resources can be found on our project website: https://coli-saar.github.io/interactive-agents.

==> applications.tex <==
\section{Applications \mareike{Rough notes}}\label{sec:applications} 
This section discusses different applications for goal-directed agents based on task characteristics described in the previous section.


\subsection{Navigation \& Object Manipulation in Physical Worlds}\label{sec:objectmanipulation}
Agents can navigate and interact with physical objects in more or less realistic simulations of physical environments described in visual or textual form, i.e. with observations in the visual or textual space. A detailed comparison between text, \twod , and \threed worlds can be found in \citet{jansen2022systematic}.

\paragraph{Visual Worlds}\label{sec:visualworlds}
Visual worlds come with observations in \twod or \threed spaces. \twod worlds are usually based on a \twod grid layout, i.e. a \twod plane with cells in discretized adjacent positions. \threed worlds range from voxel-based state representations such as the Minecraft environments to more realistic simulations of the world with various physics simulators such as AI2-Thor as underlying engine for the \tfont{\alfred} environment. Tasks usually require state changes and completion is assessed based on correspondence between final and gold states. 


%\begin{itemize}
%\item Visual worlds come with observations in \twod or \threed spaces. \twod worlds are usually based on a \twod grid layout, i.e. a \twod plane with cells in discretized adjacent positions. \threed worlds range from voxel-based state representations such as the Minecraft environments to more realistic simulations of the world with various physics simulators such as AI2-Thor as underlying engine for the \tfont{\alfred} environment. 
%\item Tasks usually require state changes and completion is assessed based on correspondence between final and gold states. 
%\end{itemize}


\paragraph{Text Worlds}\label{sec:textworlds}
 Text worlds \cite{textgames, cote2019textworld, jansen2022systematic} naturally fall into the intersection between NLP and sequential decision-making: they are virtual environments represented via textual descriptions, i.e. observations are described in natural language, and action spaces are sequences of words. They have received attention due to the fact that they can simulate \twod or \threed environments in a cheaper way, and can be used to study generalization from text to \twod or \threed spaces, e.g. \alfworld \cite{jansen2022systematic}. The existence of flexible problem generators \cite{textworld} makes them interesting for targeted studies of specific challenges (constraints on inventory size, long-range dependencies, i.e. prerequisites for solving a task have to be completed at earlier point in time, time-based events, i.e. environment state changes not triggered by agent actions).
%\begin{itemize}
%\item Text worlds \cite{textgames, cote2019textworld, jansen2022systematic}, also referred to as text games or interactive fiction games \cite{jericho} are virtual environments represented via textual descriptions, i.e. world states are described in natural language, and action spaces are sequences of words
%\item Goal achievement is usually centered around navigating partially observable environments and interacting with objects
%\item Naturally fall into the intersection between NLP and sequential decision-making
    %\item large variety in goals, complexities, and challenges
  %\item For a detailed overview on the varieties of text world tasks see \cite{textgames, cote2019textworld, jansen2022systematic}
   % \item Observation is usually a NL description of the action effect, or 'Nothing happens' if the command has no effect (valid actions), choice-based (admissible actions) vs parser-based games
     %\item Text world problems are either specified by hand, or automatically generated
     %\item \textworld \cite{textworld} is a widely used generator for text world problems. Given typed objects, typed actions types, transition function. Given the number of rooms, number of objects, number of steps, the problem generator generates a problem, i.e. a goal specification + goal state, state space (layout), and a sequence of actions required to reach the goal state. Also supports the assignment of intermediate rewards. Automatically generates textual descriptions of the environment via a CFG.
     %\item Instructions may optionally describe every action of a quest (easier), only the final action (harder), or they may force the player to figure out what to do from scratch (goal identification; hardest).
     %\item factors contributing to increased difficulty: number of steps, size of state space (number of objects + layout, e.g. rooms) 
    %\item additional challenges: constraints on inventory size, long-range dependencies, i.e. prerequisites for solving a task have to be completed at earlier point in time, time-based events, i.e. environment state changes not triggered by agent actions (e.g. triggered by biological processes such as bird hatching from egg in \scienceworld), stochasticity, random events
    %\item Text worlds have received attention due to the fact that they can simulate \twod or \threed environments in a cheaper way, and can be used to study generalization from text to \twod or \threed spaces, e.g. \alfworld
%\end{itemize}

\paragraph{PDDL Planning Problems}\label{sec:pddl}
These types of tasks are specified in the Planning Domain Description Language (PDDL), explicitly specifying action action preconditions and effects. Compared to other tasks, action and state spaces are small and usually fully observable. LLM-based agents are applied to PDDL representations directly \mareike{CITE}, or verbalized versions of the environment and observations \cite{autoplanbench}. For PDDL problems, search-based planner exist. This class of tasks is interesting to investigate the following problems: \mareike{INPUT}
%\begin{itemize}
%    \item These types of tasks are specified in the Planning Domain Description Language (PDDL), explicitly specifying action action preconditions and effects.
%    \item For PDDL problems, search-based planner exist
%    \item Compared to other tasks, action and state spaces are small and usually fully observable. 
%    \item LLM-based agents are applied to PDDL representations directly \mareike{CITE}, or verbalized versions of the environment and observations \cite{autoplanbench}.
%    \item This class of tasks is interesting to investigate the following problems:
%end{itemize}


\subsection{Digital Assistance}\label{sec:digitalassistants}
 Agents in digital worlds assist users with day-to-day tasks, and usually solve real-world problems directly useful for end users. This comprises a vast range of applications, like retrieving information, e.g. looking up information in databases, day-to-day tasks like booking travel or sending messages, analysing data, e.g. tables or images as in table or visual QA, and processing data, e.g. image editing. Some recent tasks focus on assistance in specific domains, e.g. the discovery of new chemicals \cite{chemcrow}, or fixing software bugs \cite{swebench}.\mareike{change cit.}. Agents can achieve these tasks in different ways: by interacting with external pieces of software (tools or APIs, \cref{sec:apis}), by interacting with graphical user interfaces (GUIs, \cref{sec:gui}), or by interacting with code interpreters (\cref{sec:programming}).
%\begin{itemize}
%    \item Agents in digital worlds assisting users with day-to-day tasks, and usually solve real-world problems directly useful for end users. This comprises a vast range of application, like retrieving information, e.g. looking up information in databases, day-to-day tasks like booking travel or sending messages, analysing data, e.g. tables or images as in table or visual QA, and processing data, e.g. image editing. Some recent tasks focus on assistance in specific domains, e.g. the discovery of new chemicals \cite{chemcrow}, or fixing software bugs \cite{swebench}.\mareike{change cit.}
%    \item Task differ in how the agents can achieve these tasks: by interacting with external pieces of software (tools or APIs), interacting with graphical user interfaces, interacting with code interpreters
%\end{itemize}
\subsubsection{Tool and API Orchestration}\label{sec:apis}
Agents can solve tasks by operating external pieces of software via Application Programming Interfaces (API)s, also referred to as tools\footnote{We consider APIs a special type of tools, with more complex functionality, and use both expressions interchangeably}, i.e. action spaces correspond to valid tool calls. APIs can be called in isolation, e.g. by indicating API name and arguments, or embedded in code (see \cref{sec:programming}). Observations usually correspond to the APIs return values in case execution succeeds. In case of execution failure, information about error causes can be encoded into the error messages of exceptions thrown by the APIs directly (e.g. incorrect date formatting). Recent tasks come with very large action spaces based on large amounts of APIs, and understanding the complex functionality of APIs poses one of the main challenges (select which API to use and how to call them) \mareike{CITE}. Current state-of-the-art agent methods resort to first retrieving a set of candidate APIs useful for solving a problem from the set of available APIs \mareike{CITE}, and equipping the agent with the ability to retrieve API documentation in order to decide on subsequent steps \mareike{CITE}. 
%\begin{itemize}
   % \item Agents are required to solve a task by operating external pieces of software via Application Programming Interfaces (API)s, also referred to as tools\footnote{We consider APIs a complex class of tools}, 
    %\item APIs can be called in isolation, e.g. by indicating API name and arguments, or embedded in code 
   % \item Observations usually correspond to the APIs return values in case execution succeeds. In case of execution failure, information about error causes can be encoded into the error messages of exceptions thrown by the APIs directly (e.g. incorrect date formatting)
    %\item APIs vs tools: APIs are usually more complex than simple tools like a calculator, often domain specific
     %\item actions change world states or provide information
      %\item Recent tasks come with very large action spaces based on large amounts of APIs, and understanding the complex functionality of APIs poses one of the main challenges (select which API to use and how to call them) 
      %\item Recent agent methods resort to first retrieving a set of candidate APIs useful for solving a problem from the set of available APIs \mareike{CITE}, and equipping the agent with the ability to retrieve API documentation in order to decide on subsequent steps \mareike{CITE}
%\end{itemize}


\subsubsection{GUI Interaction}\label{sec:gui}
Agents acting as digital assistants can also directly interact with graphical user interfaces (GUI) designed to be interacted with by (non-expert) users, including websites, or GUIs of mobile phone and desktop applications.  Action spaces comprise coordinate or id-based mouse and keyboard actions like \afont{click}, \afont{type}, etc. or actions for interacting with mobile screens like \afont{press}, or \afont{swipe}. Observations correspond to representations of the current state of the UI, e.g. in the form of screenshots, HTML, accessibility trees, often augmented with additional annotations like bounding boxes for indicating interactive elements in a screenshot \mareike{CITE}, or semantic labels for specific icons \mareike{CITE}. Choosing the best modality for representing observations is an active research question \mareike{CITE}, as well as how to shape the action space \mareike{CITE}. The main challenges comprise a large action space (small number of actions with large number of possible parameters, e.g. buttons to interact with), which is often tackled by pre-filtering elements to interact with \mareike{CITE}, and extracting relevant information from the observation/understanding the representation of the UI \cite{visualwebbench}, which is possibly the reason for a large number of tasks being released as trajectory-only datasets, and agents are evaluated step-by-step.
%\begin{itemize}
%\item Agents acting as digital assistants can also directly interact with graphical user interfaces (GUI) designed to be interacted with by (non-expert) users, including websites, or GUIs of mobile phone and desktop applications. 
%\item Action spaces comprise coordinate or id-based mouse and keyboard actions like \afont{click}, \afont{type}, etc. or actions for interacting with mobile screens like \afont{press}, or \afont{swipe}.
%\item Observations correspond to representations of the current state of the UI, e.g. in the form of screenshots, HTML, accessibility trees, often augmented with additional annotations like bounding boxes for indicating interactive elements in a screenshot \mareike{CITE}, or semantic labels for specific icons \mareike{CITE}. Choosing the best modality for representing observations is an active research question \mareike{CITE}, as well as how to shape the action space \mareike{CITE}
%    \item Main challenges comprise a large action space (small number of actions with large number of possible parameters, e.g. buttons to interact with), which is often tackled by pre-filtering elements to interact with \mareike{CITE}, and extracting relevant information from the observation/understanding the representation of the UI \cite{visualwebbench}, which is possibly the reason for a large number of tasks being released as trajectory-only  datasets, and agents are evaluated step-by-step.
%\end{itemize}



%\paragraph{Travel planning}
%\subsection{Question answering}\label{sec:qa}
%\paragraph{Mathematical reasoning}\label{math:qa}
\subsubsection{Code Interpreters}\label{sec:programming}
Digital agents can also directly interact with code interpreters, e.g. to execute SQL commands, or python programs. The action space is the set of all valid statements in the respective programming language. The action space can include external libraries corresponding to APIs, or directly enabling actions for interacting with a GUI. For example, \tfont{\osworld} enables an agent to navigate a GUI via a python interpreter and the python \texttt{PyAutoGUI} library. Observations directly correspond to outputs of the interpreter.
%\begin{itemize}
%    \item Agents can directly interact with a code interpreter, e.g. to execute SQL commands.
 %   \item Can use native methods in the programming languages
%   \item or specialized APIs imported to the program
 %   \item Action space is code, possibly including external libraries corresponding to APIs, or to actions for interacting with a GUI
 %   \item Observe feedback from the interpreter
%\end{itemize}

%OpenDevin


==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
We structured the current landscape of tasks for evaluating and developing goal-directed interactive agents along several dimensions useful for distinguising tasks.

==> limitations.tex <==
\section{Limitations}
\begin{itemize}
    \item Our categorization, though informed by literature, subjective
    \item No exhaustive list of all existing datasets, more prototypical
\end{itemize}

==> misc.tex <==
\subsection{Benchmarks \& Evaluation infrastructure}
\begin{itemize}
\item AgentBench \cite{agentbench}: 8 environments  (Code, Game, Web), report normalized average score, evaluate 29 LLMs
\item OpenAgents \cite{openagents}: Webinterface for Coding, API, Web agent, idea: in-the-wild evaluation of agents. Similar: Auto-GPT, SuperAGI, HuggingGPT, GPT-Engineer, LangChain, Semantic Kernal, MiniChain
\item Gentopia \cite{gentopia} platform + benchmark of tasks
\item PlanBench \cite{planbench}
\item AutoPlanBench \cite{autoplanbench}
\item OpenAGI \cite{openagi}: newly generated benchmark with image and text editing/understanding tasks
\item MINT \cite{mint}
\item LMRL-Gym \cite{lmrl}
\item AgentStudio \cite{zheng2024agentstudio}: infrastructure + in-the-wild evaluation (tool-use multi-step tasks)
\item AgentBoard \cite{ma2024agentboard}
\item Agents \cite{zhou2023agents}
\item OpenDevin
\item Dynamic evaluation: \cite{zhu2024dynamic}
\end{itemize}


==> related_work.tex <==
\section{Related Surveys}\label{sec:relatedwork}
Several recent surveys on LLM-based agents exist. %\footnote{Existing surveys on specific types of environments or specific agent applications will be mentioned in the respective parts of \cref{sec:applications}.} 
\citet{mialon2023augmented}, \citet{qin2023tool}, \citet{xi2023rise}, \citet{gao2023large}, \citet{interactivenlp}, and \citet{cheng2024exploring} provide comprehensive overviews over the single agent paradigm, with a strong focus on modeling aspects, e.g. implementations of different components in an agent system, and common applications.  \citet{xie2024large} focus on agents based on multi-modal foundation models, \citet{guo2024large}, \citet{sun2024llmbased}, and \citet{zhang2024llm} focus on the paradigm of multi-agent interaction, \citet{xu2024survey} on the application of game-playing agents. \citet{wang2024tools} provide a detailed survey on the concept of \textit{tools} for augmenting LLMs, including a detailed overview over benchmarks for tool/API-use.

Surveys by \citet{luketina2019survey}, \citet{madureira2020an} and \citet{cao2024survey} focus on the intersection of reinforcement learning and language-based environment representations. \citet{ijcai2022p770} survey methods for goal-conditioned reinforcement learning, solving the same type of tasks as focused on in this survey. The work closest to ours is \citet{peng2024survey}, which includes an overview of a broad range of applications for LLM-based agents as one part in a pipeline for holistic evaluation of LLMs. The existing surveys focus on methods and modeling aspects, and none of them provides a detailed description and comparison of the broad range of actual tasks solved by current state-of-the-art agents, which is the main contribution of our survey.




%\begin{itemize}

%\item \citet{wang2024survey} focus on llm-based agent architectures, general overview over different life areas in which agents are/could be applied. Description of different evaluation metrics, including a brief section listing benchmarks/datasets but no detailed comparison between tasks
%\item \citet{xi2023rise} take a broad view, focusing on different modules of agent architectures, brief section on task-oriented deployment without detailed discussion of datasets, discussion of different agent environments (text-based, virtual, physical) on a high level
%\item \citet{cheng2024exploring} give general survey on agent architectures, including a section on different environments (computer, gaming, code, real-world, simulation) and applications, no detailed references to datasets. Benchmark section is short, incomplete, outdated. Mention of broad potential applications.
%\item \citet{gao2023large} focus on agent architectures and their different components, discuss different domains (physical, cyber, hybrid) \item \citet{mialon2023augmented} give a detailed overview over tool-augmented LMs (tool=external module to gather information of affect virtual or physical world), different approaches for implementing such agents, and  discuss current challenges. No detailed mention of datasets
%\item \cite{qin2023tool} same as above
%\item \citet{xie2024large} survey approaches for multi-modal agents, including different evaluation methodologies, a short section on benchmarks and a short section on applications.
 %\item Multi-agents: \cite{guo2024large, sun2024llmbased}
%\item \citet{wang2024tools} provide a detailed survey on 'tools' (categories perception, action , computation), where are tools useful or not useful, survey of methods, and overview over API benchmarks
%\item \citet{interactivenlp} focus on llm-based interactive agents, focus on architectures and components. List different datasets for evaluating agent capabilites across different applications (knowledge acquisition, knowledge enhances generation, tool-in-the-loop, environment in the loop). Applications overlap with ours
%\item \citet{peng2024survey} survey applications for llm-based agents as one component in a pipeline for holistic evaluation of LLMs

%\item Interactive NLP \cite{interactivenlp}: Tool-in-the-loop vs. Environment-in-the-loop
    %\item Game-playing agents \cite{xu2024survey}
    %\item Reasoning: \cite{huang-chang-2023-towards, qiao-etal-2023-reasoning}
    %\item What's in a tool anyway? \cite{wang2024tools}
%    \item RL informed by natural language \cite{luketina2019survey}
    %\item Goal-conditioned RL \cite{ijcai2022p770}
    %\item LAW: \cite{law}
    %\item Strategic reasoning: \cite{zhang2024llm}
    %\item LLM-based RL: \cite{cao2024survey}
    %\item Coming up with challenging benchmarks: \cite{kiela-etal-2021-dynabench}
%\end{itemize}

==> tables/api_orchestration.tex <==
\begin{table*}[ht]
    \centering
    % \footnotesize
    % \setlength{\tabcolsep}{2.0pt}
    \begin{tabular}{llccccl}\toprule
                & \textbf{Tools}&\textbf{ Tools}  & \textbf{Calls}  & \textbf{Code lines} & \textbf{Rich code} & \textbf{Evaluation type}               \\
                \cmidrule{3-5}
                & & \multicolumn{3}{c}{per Task} & & \\
\makecell{\textbf{APIBench}\\ \cite{gorilla}}  & 1.6K              & 1                 & 1                       & 1                  & no               & API + Argument Matching \\
\makecell{\textbf{ToolBench}\\ \cite{toolllm}}  & 16K               & 1-3               & 1-3                     & 1-3                & no               & GPT3                    \\
\makecell{\textbf{ApiBank}\\ \cite{apibank}}   & 53                & 1-3               & 1-3                     & 1-3                & no               & Human                   \\
\makecell{\textbf{ToolTalk}\\ \cite{tooltalk}} & 28                & 1-3               & 1-3                     & 1-3                & no               & API + Argument Matching \\
\makecell{\textbf{RestBench} \\ \cite{restgpt}}  & 94                & 1-3               & 1-3                     & 1-3                & no              & Human                   \\
\makecell{\textbf{ToolAlpaca}\\ \cite{toolalpaca}} &11&1-2&1-2&1-2&no&GPT4, Human\\
\makecell{\textbf{ToolBench}*\\ \cite{oldtoolbench}} &198&1&1&1&no& Answer Matching\\
\makecell{\textbf{TaskBench}\\ \cite{taskbench}} &103& 1-8&1-8&1-8&no& \makecell[l]{API + Argument Matching,\\ Human}\\
\makecell{\textbf{Tool$^3$Eval}\\ \cite{codeact}} &15&1-4&1-12&1-30&yes&Answer Matching\\
\makecell{\textbf{ToolQA}\\ \cite{toolqa}} &13&-&-&-&no&Answer Matching\\
\addlinespace[5pt]
\makecell{\textbf{AppWorld}\\ This work}     & 410               & 1-16                 & 1-700                & 1-100                 & yes              & DB State                \\
        \bottomrule
    \end{tabular}
    \caption{\textit{Tools} in the first column refers to the number of executable tools/APIs in the respective benchmark. For ToolAlpaca, we only consider the evaluation set with executable tools. For ToolBench*, we only consider the single step tasks, as the multi-step tasks (WebShop and TableTop) focus on UI interaction and embodied decision-making rather than tool-usage. We do not report per task statistics for ToolQA, as no annotated gold solution paths are available.}
    \label{table:comparison_benchmarks}
\end{table*}

==> tables/benchmarks.tex <==
\begin{table}[t]
\resizebox{\columnwidth}{!}{
\centering
\begin{tabular}{ lcccc }\toprule
 & AgentBench & LLF-Bench & MINT & Gentopia\\
\rowcolor{tablegrey}
PDDL &  &  &  & $\bullet$\\
Code & $\bullet$ &  & $\bullet$ & $\bullet$\\
\rowcolor{tablegrey}
QA & $\bullet$ &  & $\bullet$ & \\
CG & $\bullet$ &  &  & \\
\rowcolor{tablegrey}
Puzzle & $\bullet$ &  &  & \\
TG & $\bullet$ & $\bullet$ & $\bullet$ & \\
\rowcolor{tablegrey}
UI & $\bullet$ &  &  & \\
Bandits &  & $\bullet$ &  & \\
\rowcolor{tablegrey}
Math &  &  & $\bullet$ & $\bullet$\\
\bottomrule
\end{tabular}
}
\caption{ Current agent benchmarks (x-axis) evaluate agents across a range of different tasks reflecting different application scenarios (y-axis). }
\label{tab:benchmarks}
\end{table}

==> tables/coarse.tex <==
\begin{table*}[t]
\resizebox{\textwidth}{!}{
\centering
\begin{tabular}{ ccccccc }\toprule
 \textbf{ Task }  &  \textbf{ Example DS }  & \multicolumn{  2  }{c}{ \textbf{ World State } } & \multicolumn{  2  }{c}{ \textbf{ Action Space } } &  \textbf{ Uncertainty } \\
Task & Example DS & \rotatebox[]{80}{\ \ Changeable\ \ } & \rotatebox[]{80}{\ \ Observable\ \ } & No. Actions & No. Arguments & \\
PDDL Planning & Blocksworld & \checkcolor{\ding{51}} & \includegraphics[height=2.5ex]{images/full_worldstate.png} & Small & Limited & \\
Bandits & LLF-Bench & \crosscolor{\ding{55}} & \includegraphics[height=2.5ex]{images/partial_worldstate.png} & Small & - & \\
Text games & \alfworld & \checkcolor{\ding{51}} & \includegraphics[height=2.5ex]{images/explore_worldstate.png} & Small & Limited & \\
Minecraft &  & \checkcolor{\ding{51}} & \includegraphics[height=2.5ex]{images/partial_worldstate.png} & Small & Limited & \\
API orchestration & \appworld & \checkcolor{\ding{51}} & \includegraphics[height=2.5ex]{images/explore_worldstate.png} & Large & Unlimited & \\
UI interaction & WebArena & \checkcolor{\ding{51}} & \includegraphics[height=2.5ex]{images/explore_worldstate.png} & Small & Large & \\
Travel Planning &  & \checkcolor{\ding{51}} & \includegraphics[height=2.5ex]{images/partial_worldstate.png} & Small & Unlimited & \\
Question Answering & HotpotQA & \crosscolor{\ding{55}} & \includegraphics[height=2.5ex]{images/partial_worldstate.png} & Small & Unlimited & \\
Mathematical reasoning &  & \crosscolor{\ding{55}} & \includegraphics[height=2.5ex]{images/partial_worldstate.png} & Small & Unlimited & \\
\bottomrule
\end{tabular}
}
\caption{ Overview over agent tasks. }
\label{ t:coarse }
\end{table*}
